Flatness Based Control of an Industrial Robot Joint Using Secondary Encoders

Due to their compliant structure, industrial robots without precision-enhancing measures are only to a limited extent suitable for machining applications. Apart from structural, thermal and bearing deformations, the main cause for compliant structure is backlash of transmission drives. This paper proposes a method to improve trajectory tracking accuracy by using secondary encoders and applying a feedback and a flatness based feed forward control strategy. For this purpose, a novel nonlinear, continuously differentiable dynamical model of a flexible robot joint is presented. The robot joint is modeled as a two-mass oscillator with pose-dependent inertia, nonlinear friction and nonlinear stiffness, including backlash. A flatness based feed forward control is designed to improve the guiding behaviour and a feedback controller, based on secondary encoders, is implemented for disturbance compensation. Using Automatic Differentiation, the nonlinear feed forward controller can be computed in a few microseconds online. Finally, the proposed algorithms are evaluated in simulations and experimentally on a real KUKA Quantec KR300 Ultra SE.

==> doc/sec_control_design.tex <==
\section{Controller Design}

We propose a model-based feed forward term to account for the dynamic system and a feedback control law for compensation of unknown disturbances and model errors. 
In Fig.~\ref{fig:closed-loop-model} and Fig.~\ref{fig:exact_linear_feedback} two different architectures for feed forward control are presented. Both of them contain a feed forward term, a feedback controller and trajectory planning. First of all, we discuss the common elements of both architectures and then we will explain the differences in their integration.
\begin{figure}
	\centering
	\resizebox{\columnwidth}{!}{%
	\input{figs/closed_loop_tikz_v2}}
	\caption{Controller design with feed forward and feedback control}
	\label{fig:closed-loop-model}
\end{figure}

\begin{figure}
	\centering
	\resizebox{\columnwidth}{!}{%
	\input{figs/exact_linearization_tikz_v2}}
	\caption{Controller design with exact linearization}
	\label{fig:exact_linear_feedback}
\end{figure}

\subsection{Control architectures}
The trajectory planning generates the reference signals, i.e. the link angle $ q_{R} $ and its derivatives of a desired trajectory. A motor torque $\tau_M$ is applied to the robot and the link angle $q$ and the link velocity $\dot{q}$ are the control variables of the feedback controller. The link angle $q$ can be measured directly using SE and the motor velocity $\dot{\theta}$ can be measured using the motor resolver. For both sensors, noise is neglected. However, we implement the velocity controller on the link side, using $\dot{q}$, and neglect the resolver. Considering elastic joints, it is difficult to precisely calculate the motor reference speed, since the equation $q_i = u_i \theta_i$ is only valid for rigid joints. A presice calculation of the motor reference speed requires the full, nonlinear stiffness model and is thus vulnerable to modeling errors. Therefore, we implement the feedback controller exclusively on the link side. Both, the position and velocity controller and realized as P controllers. The position controller is given by
\begin{equation}
\dot{q}_{C} =  K_{p} \, (q_{R}  - q),
\label{eq: pos_controller}
\end{equation}
with the proportional position gain $K_{p}$ and the controller speed $\dot{q}_{C}$. The velocity controller using the proportional speed gain $K_{v}$ has the form
\begin{equation}
 u_{vel} = \tau_{FF} + K_{v} \, \left(  \dot{q}_{C} + \dot{q}_{R} - \dot{q} \right).  
\end{equation}

Regarding the feed forward term, there are two different architectures, as presented in Fig.~\ref{fig:closed-loop-model} and Fig.~\ref{fig:exact_linear_feedback}. The design in Fig.~\ref{fig:closed-loop-model} is referred to as flatness-based feed forward control, whereas the structure in Fig.~\ref{fig:exact_linear_feedback} is known as exact linearization. Depending on the literature, both of them are called computed torque control \cite{Moberg2008}. To reduce the risk of confusion, we will avoid the term computed torque control in this contribution. The flatness based design is explained in detail in Sec.~\ref{sec:flatness} and computes the feed forward torque independently of the current states. It relies only on the reference trajectory and its derivatives and therefore, it can potentially be computed offline. As a consequence, it is robust to any measurement noise. The flatness based architecture is independent of the feedback control and therefore, the feedback control is not delayed or modified in any sense. It contains the disadvantage of a potentially less precise model since it relies on the reference trajectory rather than the state trajectory. However, it is possible to include some online measurements to improve the model accuracy. The inertia matrix, gravity, Coriolis and centripetal terms are based on measurements rather than on the reference trajectory. 

The exact linearization architecture, as presented in Fig.~\ref{fig:exact_linear_feedback}, attempts to eliminate the nonlinear robot dynamics in an inner loop and therefore control a simple, linear system with the feedback controller. A detailed explanation is given in \cite{Spong1987}. Basically, the feedback controller computes an angular acceleration for a dynamic inversion-based controller in order to compensate the nonlinear dynamics. 
% modified link angle derivative $ \ddot{\mathbf{q}}_{i}^{*} $. Based on the modified angle derivative, a motor torque is computed using the inverse nonlinear model. \\

Its advantage is that the feedback controller is automatically adjusted to the current robot state. Disadvantages are a necessity of a fast computation of the dynamic model in the inner loop and a potential time delay of the feedback control. In \cite{Nguyen-Tuong2008} both designs are compared and the flatness-based architecture outperforms the exact linearization structure with several feed forward models regarding the achieved trajectory accuracy. The authors argue, that the main advantage of a feed forward structure compared to exact linearization is the direct and non-delayed effect of the feedback control. Based on these empirical results, we decide to apply a flatness-based architecture rather than exact linearization.
% (Thanks to Automatic-Differentiation and a completely differentiable model, the proposed feed forward control can be computed online  very fast, i.e. a few microseconds. As a result, it is suited for a exact linearization formulation although its validation requires further research and stays beyond the scope of this paper. (\textbf{Comment}: This can be skipped)). \\
Usually, the exact linearization module does not account for joint elasticity and therefore, the inner loop reduces to a double integrator. The main idea, to apply the inverse of the model, remains the same in the flatness-based feed forward and the exact linearization case. Assume a model inverse of the robot is given by the following form
\begin{equation}
    % \tau_M = f( q_{U}, \dot{q}_{U}, \cdots, \frac{d^D{q}_{U}}{d t^D} ),
    \tau_M = f( q_{U}, \dot{q}_{U}, \cdots, {q}^{(D)}_{U} ),
    \label{eq:model_inverse}
\end{equation}
with an input angle $q_{U}$ and its derivatives. We define the derivative as ${q}^{(D)} = \frac{d^D{q}}{d t^D}$. In the flatness-based architecture, we set $q_{U} = q_{R}$. In the exact linearization formulation, we apply
\begin{equation}
    {q}^{(D)}_{U} = {q}^{(D)}_{R} + {q}^{(D)}_{C},
\end{equation}
with the feedback control variable ${q}^{(D)}_{C}$. With an elastic joint the model derivative order is $D = 4$ and without an elastic joint $D = 2$ \cite{Moberg2008}. So, for a model without elastic joints we obtain
\begin{equation}
    \ddot{q}_{U} = \ddot{q}_{R} + \ddot{q}_{C},
\end{equation}
and for a model with elastic joints we get
\begin{equation}
    {q}^{(4)}_{U} = {q}^{(4)}_{R} + {q}^{(4)}_{C}.
\end{equation}

 In the exact linearization case it is beneficial to apply the highest input derivative. Note that the output of the velocity controller $u_{C}$ depends on the architecture. In the flatness-based case, it is equal to the motor control torque, i.e. $u_{C} = \tau_C$. In the exact linearization case, it computes the control input of the inverse dynamics model, i.e. $ u_{C} = {q}^{(D)}_{C}$. In the following, we derive the flatness-based module and thus estimate \eqref{eq:model_inverse}. \\
 

% In the following the control design for each joint is presented. In Fig.~\ref{fig:closed-loop-model} the feedback structure of the control loop is shown together with the trajectory planning and the feed forward control. The trajectory planning generates the reference signals, i.e. the motor speed $ \dot{\theta}_{R} $ and the link angle $ q_{R} $ of a desired trajectory. The feed forward torque $ \tau_{FF} $ is calculated based on the reference link angle $ q_{R} $. Together with the control torque $ \tau_{C} $, the input torque $ \tau_{M} $ for the motor is build.
% The link angle $q$ and the motor speed $\dot{\theta}$ are the control variables of the feedback controller. The link angle $q$ can be measured directly using SE and the motor velocity $\dot{\theta}$ is measured using the motor resolver. For both sensors, noise is neglected. The speed controller is implemented as a PI controller and the position controller is realized with a P controller.
% The measured signals are the motor speed $ \dot{\varphi}_{M} $ and the link angle $ \varphi_{A} $. 
% The arm angle $\varphi_A$ is the primary control variable. Additionally, in the inner loop of the controller, see Fig.~\ref{fig:closed-loop-model}, the motor speed $\dot{\varphi}_M$ serves as control variable. Both, $\varphi_A$ and $\dot{\varphi}_M$, can be measured.
% In case of deviations of the reference signals  $ \dot{\varphi}_{RM} $ and $ \varphi_{RA} $  a control torque  $ \tau_{C} $ is implied by the feedback controller. Here, the output signal of the position controller is concurrent the input signal of the subordinate speed controller. 
 


% \subsection{Exact linearization Based Control}
% \label{sec:exact_linearization}









\subsection{Flatness Based Feed Forward Control}
\label{sec:flatness}

The main task of the feed forward control law is to achieve a good guiding behavior, whereby the feedback control law can be applied exclusively for the compensation of disturbances and model uncertainties. For the design of the feed forward control, the inverse nonlinear model of the robot link is used. Therefore, the nonlinear model \eqref{eq:robotdynamics} and \eqref{eq:robotdynamics2} is solved for the motor torque $ \tau_{M} $, valid for each link, in the form
\begin{align}
\tau_{M} = J \, \ddot{\theta} +  \frac{M \, \ddot{q} + \tau_I + \tau_{CC} + g + \tilde{\tau}_{F}(\dot{q})}{u}.
% \, \left(M(q) \, \ddot{q} + \tau_{CC} + g(q) + \tilde{\tau}_{F}(\dot{q})\right).
\label{eq:motor_torque}
\end{align}

Equation \eqref{eq:motor_torque} describes the motor torque applied in a specific operating point. For a good guiding behavior, i.e. $q = q_R$, the motor position is set to the reference position, i.e. $\theta = \theta_R$ and $\tau_{M} = \tau_{FF}$ is applied. It follows % Therefore, a formulation for $\tau_{M}$ has been obtained by \eqref{eq:motor_torque}, which relies on static parameters, the link angle $q$ and its derivatives only.  
\begin{align}
\tau_{FF} = J \, \ddot{\theta}_R +  \frac{M \, \ddot{q}_R + \tau_I + \tau_{CC} + g + \tilde{\tau}_{F}(\dot{q}_R)}{u} .
% \left(M(q_R) \, \ddot{q}_R + \tau_{CC} + g(q_R) + \tilde{\tau}_{F}(\dot{q}_R)\right). 
\label{eq:motor_torque_ff}
\end{align}

In order to solve \eqref{eq:motor_torque_ff}, we need to use the model equations to substitute all variables, such as $\ddot{\theta}_R$, with a function of $q_R$. The following section shows how to determine each term in \eqref{eq:motor_torque_ff}.

\begin{enumerate}
\item The continuous differentiable friction torque $ \tilde{\tau}_{F}(\dot{q_R}) $ is defined in \eqref{eq:mod_friction_app}.
\item The Coriolis and centripetal torques are summarized for each link in $\tau_{CC,i}$ with
\begin{equation}
    \tau_{CC,i} = \sum_{j = 1}^{N} c_{i,j} \, q_j, \qquad i \neq j.
\end{equation}
Note that $\tau_{CC,i}$ is not a function of $q_i$. For the sake of simplicity, index $i$ is omitted in the following since all variables and parameters in the flatness based control refer to the same link index $i$. $\tau_{CC}$ can be calculated using the kinematics of the robot.
\item The link inertia $M$ and the link gravity torque $g$ can be obtained from the kinematics of the robot. We summarize the inertia torques caused by other links in the inertia torque $\tau_{I,i}$
\begin{equation}
    \tau_{I,i} = \sum_{j = 1}^{N} M_{i,j} \, \ddot{q}_{R, j}, \qquad i \neq j.
\end{equation}
\item The motor angle $\theta$ is substituted in \eqref{eq:motor_torque_ff} using the inverse nonlinear stiffness model. We use the torsion angle $ \Delta q $ as defined in \eqref{eq:torsion_diff_angle} and solve for $\theta$ 

\begin{equation}
 \theta = u \, ( \Delta q + q ).
\end{equation}

The torsion angle $\Delta q$ is substituted using the inverse, continuous stiffness model \eqref{eq:mod_stiff_app} leading to

\begin{equation}
 \theta = u \, \left( \frac{\tilde{\tau}_{E}}{c_{TR}} + \frac{2 \, \Phi_{B}}{1+e^{-s_{E} \, \tilde{\tau}_{E}}} - \Phi_B + q \right).
\end{equation}

The elastic torque is substituted using the sum of torques of the link. Furthermore, we set $\theta = \theta_R $ and $q = q_R$ and obtain

\begin{equation} \label{eq:feedforward}
\begin{split}
 \theta_R &= u \, ( \frac{M \, \ddot{q}_R + \tau_I + \tau_{CC} + g + \tilde{\tau}_{F}(\dot{q}_R)}{c_{TR}} \\
 &\qquad + \frac{2 \, \Phi_{B}}{1+e^{-s_{E} \, \left( M \, \ddot{q}_R + \tau_I + \tau_{CC} + g + \tilde{\tau}_{F}(\dot{q}_R) \right)}} \\ &\qquad - \Phi_B + q_R ).
\end{split}
\end{equation}

Obtaining the second derivative of \eqref{eq:feedforward}, i.e. $ \ddot{\theta}_{R} = \frac{\diff^2 \theta_{R}}{\diff t^2} $, completes the solution for $\tau_{FF}$  in \eqref{eq:motor_torque_ff}.  \textit{MATLAB Symbolic Math Toolbox} was used for solving the equations. %In order the get a fast on-line implementation, a numerical approximation of the solution, created with \textit{matlabFunctionBlock()}. 
It should be pointed out, that due to the pre-computation of the solution using AD, the run time of the feed forward calculation requires only a few microseconds. This is only possible because the continuous formulation of the model allows to use AD tools. For safety and implementation reasons, we manually edited the flatness based feed forward control as presented in Appendix \ref{app:code}.
\end{enumerate}

% \subsection{Manual Adjustments of the Feed Forward Control}

% For safety and implementation reasons, we manually edited the flatness based feed forward control as follows.
% \begin{enumerate}
%\item We translated the code from \textit{MATLAB} to \textit{c++} language. The code is supplemented in Appendix \ref{app:code}.
%\item We limited all exponential functions $exp( \cdot ) \leq 1e30$ in order to avoid Not-A-Number and infinity errors when using division. 
% \item We limited the feed forward torque $\tau_{LIM}$ as well as its maximum change rates $\dot{\tau}_{LIM}$ according to Tab.~\ref{tab:tableparameters}.
% \item We low pass filtered $\tau_{FF}$ in order to avoid step changes of the torque due to Coulomb friction and backlash at the start of the experiments.
% \item The single link movement of axis 1 allows to omitted both, the gravity torque and the Coriolis and centripetal torques.
% \end{enumerate}
	

==> doc/sec_results.tex <==

\section{Experimental Results}

The presented feed forward and feedback control laws are validated on a \textit{KUKA Quantec KR300 Ultra SE} robot pictured in Fig.~\ref{fig:robot_picture}. %While the mechanical system is not modified, a custom made controller from \textit{B\&R Automation} is applied. 
The hardware and robot operating system are based on components from \textit{KUKA} and  industrial supplier \textit{B\&R Automation}. The \textit{B\&R Automation} robot operating system allows to implement the control algorithms as presented in  Fig.~\ref{fig:closed-loop-model}.
% the presented control algorithms without modifications with respect to Fig.~\ref{fig:closed-loop-model}.
% The above mentioned algorithms where implemented in the B&R real time system environment.
% This custom tailored electronics enables a profound control of the power electronics, the sensor integration and the robot programming. 
Except for the velocity control which runs in a task class of $0.2$~$ms$, all other presented algorithms run in a task class of $0.8$~$ms$. On the $6$ joint manipulator, SE are mounted on joints $1$, $2$ and $3$ and utilized for position control as illustrated in Fig.~\ref{fig:closed-loop-model}. The motor encoders of the first three joints are used for velocity control only. Joints $4$, $5$ and $6$ are not equipped with SE and apply motor encoders for position and velocity control. We focus our results on joints $1$, $2$ and $3$ since these joints can directly measure elastic joint effects and therefore can validate the core contributions of this work.

\begin{figure}
    \centering
    \includegraphics[width = 0.4\textwidth]{figs/robo_picture_2.jpg}
    \caption{\textit{KUKA Quantec KR300 Ultra SE}}
    \label{fig:robot_picture}
\end{figure}

As experimental scenario, a cartesian full robot movement was chosen. The movement of joints $1$, $2$ and $3$ can be measured using the same SE applied for position control. Each SE achieves an accuracy of $0.035 \ \mathrm{deg}$. All experiments are carried out on the cold robot, where both gearboxes and motors have approximately a temperature of $24.7$\textdegree{}, measured before and after the experiments. This leads to a significant and nonlinear friction in the base joints. The experiment has been carried out $10$ times in a row and the measurements are representative and reproducible.

The reference trajectory of the movement is shown in Fig.~\ref{fig:reference_plot_cart}. The cartesion movement starts in a homing position, as presented in Fig.~\ref{fig:robot_picture}, and performs a planar eight-knot movement. The trajectory is based on the Lemniscate of Gerono, which can be parametrized as

\begin{align}
    x &= 0.8m \, cos( \varphi ), \\
    y &= 0.8m \, sin( \varphi ) \, cos( \varphi ) \nonumber.
\end{align}

We apply both, a cartesian space and a joint space filter to make the trajectory in $7^{th}$ order continuously differentiable. In order to explicitly test effects of backlash, lost-motion and Coulomb friction we chose a movement with several changes in direction and parts with link velocities close to zero. The joint space reference trajectory is shown in Fig.~\ref{ex_reference_plot_joint_v1}.

\begin{figure}
	\centering
	\setlength\fheight{3.5cm}
	\setlength\fwidth{7cm}
	\input{figs/ex_reference_plot_cart_v1}
	\caption{Cartesion TCP trajectory. Reference and FB-FF.}
    \label{fig:reference_plot_cart}
\end{figure}

\begin{figure}
	\centering
	\setlength\fheight{3.5cm}
	\setlength\fwidth{7cm}
	\input{figs/ex_reference_plot_joint_v1}
	\caption{Joint space reference trajectory with velocity and acceleration for each joint}
    \label{fig:reference_plot_joint}
\end{figure}

Besides the reference trajectory, Fig.~\ref{fig:reference_plot_cart} also presents the main result: the actual movement of the link measured using only a feedback control and the movement of the same trajectory using both, feedback and feed forward control. This improvement is also shown in Fig.~\ref{fig:error_plot}, which presents the angular displacement $q_{\Delta, 1} = q_{R,1} - q_1 $ of link $1$ in both cases. It can be seen, that an improvement of $ 85.8 \ \% $ regarding angular accuracy can be achieved, improving from $1.61 \ \mathrm{deg}$ to $ 0.23 \ \mathrm{deg}$. Considering a $1500 \ mm$ long lever, this results in an end-effector accuracy improvement from $42.1\ mm$ to $ 6 \ mm$.

The measured motor torques are illustrated in Fig.~\ref{fig:torque_plot}. The figure shows both cases, the feedback control with and without feed forward control. For comparison, we added the pure feed forward torque in the same plot. Note that there is almost no difference between the pre-computed feed forward torque and the executed feedback and feed forward torque. Consequently, the feedback control applied almost no changes to the feed forward torque. We conclude, that our approach is accurate enough to capture all relevant robot dynamics. In other words, if there was a significant gap between model and real robot, the feedback control would have intervened, which did not happen.

In a critical review we find that there is a considerable difference between simulation and real robot results. As remarked before, this is mainly due to model errors, sensor noise and external disturbances which are neglected in the presented simulation. The gap between simulation and experimental results vanishes if, for example, model errors are included in the simulation. However, in this case the difference between flatness based and standard control also vanishes, since both feed forward control algorithms can not account for model errors. Reviewing the feed forward torque comparison, Fig.~\ref{fig:sim_ff_torque} demonstrates that the standard control already captures the major robot dynamics. A similar result is found in the angular displacement simulation in Fig.~\ref{fig:sim_error}, where the flatness based control is of course better, but the standard feed forward control nevertheless achieves an accuracy of $ 0.06 \ \mathrm{deg}$. We find this result is surprising, since the standard control does not model any joint elasticity. To be clear, the flatness based control is equal or better in all categories. The computed feed forward torque difference is just not significant compared to other error sources like noise, model errors and external disturbances.

The main advantages of flatness based control originate from a different perspective. First of all, note in Fig.~\ref{fig:sim_elastic_torque} the gearbox oscillations which are created due to backlash and Coulomb friction. These oscillations feature a considerable amplitude of $ 1500 \  \mathrm{Nm}$. Using an accurate flatness based control eliminates these oscillations. 

Second, all in all only the combined performance of feed forward and feedback control is relevant. It is well-known, that a motor-side velocity controller can achieve a greater bandwidth than a link-side velocity controller. However, for implementing a motor-side velocity controller the calculation of the motor reference velocity $\dot{\Theta}_{R,1} $ is non-trivial. Usually, elastic joints are neglected and a incorrect reference is applied, i.e. $\dot{\Theta}_{R,1} = u \, \dot{q}_{R,1}$. In order to calculate correctly, the full non-linear model dynamics \eqref{eq:feedforward} need to be taken into account. For a rigid joint model, like the standard control, it is impossible to calculate the correct motor reference velocity since this elastic joint effect is neglected in the first place. The flatness based control is able to fulfil this task and requires only a few microseconds computation time due to AD. Therefore, the flatness based control enables a better feedback velocity controller.

% We compare the measured torques with the pre-computed flatness based feed forward torque in Fig.~\ref{fig:torque_plot}. The presented model is precise enough that there is almost no difference between the FC-FF torque and the combined torque from FB-FF and FB-C. Using this control design, the feedback control has almost no influence when combined with the flatness based model.

\begin{figure}
	\centering
	\setlength\fheight{3.5cm}
	\setlength\fwidth{7cm}
	\input{figs/ex_error_plot_B_v3}
	\caption{Measured angular displacement $q_{\Delta,i}$ of each link $i$  with flatness based feed forward (FB-FF) and nonlinear feed forward (N-FF).}
    \label{fig:error_B_plot}
\end{figure}

\begin{figure}
	\centering
	\setlength\fheight{3.5cm}
	\setlength\fwidth{7cm}
	\input{figs/ex_error_plot_A_v3}
	\caption{Measured angular displacement $q_{\Delta,i}$ of each link $i$  with flatness based feed forward (FB-FF), feedback control (FB-C) and enhanced feedback control (EFB-C).}
    \label{fig:error_A_plot}
\end{figure}

\begin{figure}
	\centering
	\setlength\fheight{3.5cm}
	\setlength\fwidth{7cm}
	\input{figs/ex_torque_meas_v2}
	\caption{Measured motor torque $\tau_{M,i}$ of each link $i$ with feedback control (FB-C) and feed forward torque (FB-FF). The stand-alone FB-FF torque executed is presented for comparison.}
    \label{fig:torque_plot}
\end{figure}


\section{Conclusion}
It was shown that the derived flatness based feed forward control is capable of utilizing complex, nonlinear dynamical model of the joint flexibility and improving the position precision significantly. Joint backlash and lost-motion can be modeled using a novel nonlinear, continuous differentiable function. This enables standard AD tools, which allow fast run time cycles since the flatness forward controller only requires a few microseconds of computation time online. However, computation of the flatness based control within microseconds is not required when only a-priori knowledge is used. In future works, we consider online parameter identification as well as feedback linearization techniques. Both require very fast online computations. In this paper, we show that this requirement can be fulfilled. Parameter identification during run time enables model adaption to time-varying parameters, such as temperature depended joint friction. Furthermore, an extension of the complete robot movement has to be evaluated experimentally.

\textcolor{red}{Results: axis 2, torque diff but no angular error - probably hydraulics and gravity model errors, and minimal movement amplitude of axis 2, therefore minimal torques, therefore minimal errors, and asymmetrical friction, outlook, and sensor resolution limitations.
Outlook: \begin{itemize}
    \item Nonlinear System Identification
    \item Hydraulic Modelling, asymetrical Friction
\end{itemize}
Appendix:
\begin{itemize}
    \item Robot Parameters
\end{itemize}}

% \section{Intern Comments}

% Influence of flatness based Control
%  - almost no improvement regarding accuracy
%  - potential reduction of gearbox elasticity torque oscillations
%  - correct combination with arm-based PD control instead of PPI
%  - no comparision between exact linearisation and feedforward yet
%  - single axis only
